Wright's First-Order Logic of Strict Finitism

A classical reconstruction of Wright's first-order logic of strict finitism is presented. Strict finitism is a constructive standpoint of mathematics that is more restrictive than intuitionism. Wright sketched the semantics of said logic in Wright (Realism, Meaning and Truth, chap 4, 2nd edition in 1993. Blackwell Publishers, Oxford, Cambridge, pp.107-75, 1982), in his strict finitistic metatheory. Yamada (J Philos Log. https://doi.org/10.1007/s10992-022-09698-w, 2023) proposed, as its classical reconstruction, a propositional logic of strict finitism under an auxiliary condition that makes the logic correspond with intuitionistic propositional logic. In this paper, we extend the propositional logic to a first-order logic that does not assume the condition. We will provide a sound and complete pair of a Kripke-style semantics and a natural deduction system, and show that if the condition is imposed, then the logic exhibits natural extensions of Yamada (2023)'s results.

==> figure1.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=small] (0) at (-5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_0$}] (2) at (-4, 0) {};
		\node [style=small] (4) at (-3, 4) {};
		\node [style=small] (5) at (-2.5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_1$}] (6) at (-1.5, 0) {};
		\node [style=small] (7) at (-0.5, 4) {};
		\node [style=small] (8) at (0, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_2$}] (9) at (1, 0) {};
		\node [style=small] (10) at (2, 4) {};
		\node [style=small] (11) at (2.5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_3$}] (12) at (3.5, 0) {};
		\node [style=small] (13) at (4.5, 4) {};
		\node [style=small, label={[font=\tiny]left:$r_*$}] (17) at (-3, -2) {};
		\node [style=small] (23) at (-4.25, 1) {};
		\node [style=small] (24) at (-3.75, 1) {};
		\node [style=small] (25) at (-1.75, 1) {};
		\node [style=small] (26) at (-1.25, 1) {};
		\node [style=small] (27) at (-4.5, 2) {};
		\node [style=small] (28) at (-3.5, 2) {};
		\node [style=small] (29) at (-4.75, 3) {};
		\node [style=small] (30) at (-3.25, 3) {};
		\node [style=small] (31) at (-2.25, 3) {};
		\node [style=small] (32) at (-0.75, 3) {};
		\node [style=small] (33) at (-2, 2) {};
		\node [style=small] (34) at (-1, 2) {};
		\node [style=small] (35) at (0.25, 3) {};
		\node [style=small] (36) at (1.75, 3) {};
		\node [style=small] (37) at (0.5, 2) {};
		\node [style=small] (38) at (1.5, 2) {};
		\node [style=small] (39) at (0.75, 1) {};
		\node [style=small] (40) at (1.25, 1) {};
		\node [style=small] (41) at (3.25, 1) {};
		\node [style=small] (42) at (3.75, 1) {};
		\node [style=small] (43) at (3, 2) {};
		\node [style=small] (44) at (4, 2) {};
		\node [style=small] (45) at (2.75, 3) {};
		\node [style=small] (46) at (4.25, 3) {};
		\node [style=none] (93) at (-4, 4.5) {{\tiny $\nabla_0$}};
		\node [style=none] (94) at (-1.525, 4.5) {{\tiny $\nabla_1$}};
		\node [style=none] (95) at (0.975, 4.5) {{\tiny $\nabla_2$}};
		\node [style=none] (96) at (3.475, 4.5) {{\tiny $\nabla_3$}};
		\node [style=none] (97) at (-6.5, 4.5) {{\tiny Depth}};
		\node [style=none] (98) at (-6.5, 4) {};
		\node [style=none] (99) at (-6.5, 3) {};
		\node [style=none] (100) at (-6.5, 2) {};
		\node [style=none] (101) at (-6.5, 1) {};
		\node [style=none] (102) at (-6.5, 0) {};
		\node [style=none] (103) at (-6.5, 0) {{\tiny $0$}};
		\node [style=none] (104) at (-6.5, 1) {{\tiny $1$}};
		\node [style=none] (105) at (-6.5, 2) {{\tiny $2$}};
		\node [style=none] (106) at (-6.5, 3) {{\tiny $3$}};
		\node [style=none] (107) at (-6.5, 4) {{\tiny $4$}};
		\node [style=none] (108) at (6, 2) {$\cdots$};
		\node [style=none] (109) at (3, -1.5) {$\cdots$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [style=semithick] (0) to (2);
		\draw [style=semithick] (2) to (4);
		\draw [style=semithick] (0) to (4);
		\draw [style=semithick] (5) to (6);
		\draw [style=semithick] (6) to (7);
		\draw [style=semithick] (5) to (7);
		\draw [style=semithick] (8) to (9);
		\draw [style=semithick] (9) to (10);
		\draw [style=semithick] (8) to (10);
		\draw [style=semithick] (11) to (12);
		\draw [style=semithick] (12) to (13);
		\draw [style=semithick] (11) to (13);
		\draw [style=semithick] (2) to (17);
		\draw [style=semithick] (17) to (6);
		\draw [style=semithick] (17) to (9);
		\draw [style=semithick] (17) to (12);
		\draw [style=semithick] (23) to (24);
		\draw [style=semithick] (27) to (28);
		\draw [style=semithick] (29) to (30);
		\draw [style=semithick] (31) to (32);
		\draw [style=semithick] (33) to (34);
		\draw [style=semithick] (25) to (26);
		\draw [style=semithick] (35) to (36);
		\draw [style=semithick] (37) to (38);
		\draw [style=semithick] (39) to (40);
		\draw [style=semithick] (41) to (42);
		\draw [style=semithick] (43) to (44);
		\draw [style=semithick] (45) to (46);
	\end{pgfonlayer}
\end{tikzpicture}


==> figure2.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=small] (0) at (-5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_0$}] (2) at (-4, 0) {};
		\node [style=small] (4) at (-3, 4) {};
		\node [style=small] (5) at (-2.5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_1$}] (6) at (-1.5, 0) {};
		\node [style=small] (7) at (-0.5, 4) {};
		\node [style=small] (8) at (0, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_2$}] (9) at (1, 0) {};
		\node [style=small] (10) at (2, 4) {};
		\node [style=small] (11) at (2.5, 4) {};
		\node [style=small, label={[font=\tiny]right:$r_3$}] (12) at (3.5, 0) {};
		\node [style=small] (13) at (4.5, 4) {};
		\node [style=small, label={[font=\tiny]left:$r_*$}] (17) at (-3, -2) {};
		\node [style=small] (23) at (-4.25, 1) {};
		\node [style=small] (24) at (-3.75, 1) {};
		\node [style=small] (25) at (-1.75, 1) {};
		\node [style=small] (26) at (-1.25, 1) {};
		\node [style=small] (27) at (-4.5, 2) {};
		\node [style=small] (28) at (-3.5, 2) {};
		\node [style=small] (29) at (-4.75, 3) {};
		\node [style=small] (30) at (-3.25, 3) {};
		\node [style=small] (31) at (-2.25, 3) {};
		\node [style=small] (32) at (-0.75, 3) {};
		\node [style=small] (33) at (-2, 2) {};
		\node [style=small] (34) at (-1, 2) {};
		\node [style=small] (35) at (0.25, 3) {};
		\node [style=small] (36) at (1.75, 3) {};
		\node [style=small] (37) at (0.5, 2) {};
		\node [style=small] (38) at (1.5, 2) {};
		\node [style=small] (39) at (0.75, 1) {};
		\node [style=small] (40) at (1.25, 1) {};
		\node [style=small] (41) at (3.25, 1) {};
		\node [style=small] (42) at (3.75, 1) {};
		\node [style=small] (43) at (3, 2) {};
		\node [style=small] (44) at (4, 2) {};
		\node [style=small] (45) at (2.75, 3) {};
		\node [style=small] (46) at (4.25, 3) {};
		\node [style=none] (53) at (-3.575, -1) {};
		\node [style=none] (55) at (-4.325, 1.075) {};
		\node [style=none] (57) at (-1.575, 0) {};
		\node [style=none] (58) at (-3.675, 1.075) {};
		\node [style=none] (59) at (-4.075, 0) {};
		\node [style=none] (60) at (-1.825, 1.075) {};
		\node [style=none] (61) at (-1.175, 1.075) {};
		\node [style=none] (62) at (-4.575, 1.925) {};
		\node [style=none] (66) at (0.675, 1.075) {};
		\node [style=none] (67) at (1.325, 1.075) {};
		\node [style=none] (68) at (0.425, 1.925) {};
		\node [style=none] (69) at (0.425, 2.075) {};
		\node [style=none] (72) at (-4.575, 2.075) {};
		\node [style=none] (73) at (-0.925, 2.075) {};
		\node [style=none] (74) at (0.925, 0) {};
		\node [style=none] (77) at (3.425, 0) {};
		\node [style=none] (78) at (3.175, 1.075) {};
		\node [style=none] (79) at (3.825, 1.075) {};
		\node [style=none] (80) at (2.925, 1.925) {};
		\node [style=none] (81) at (2.925, 2.075) {};
		\node [style=none] (82) at (4.075, 2.075) {};
		\node [style=none] (83) at (2.675, 2.925) {};
		\node [style=none] (84) at (2.675, 3.075) {};
		\node [style=none] (85) at (4.325, 3.075) {};
		\node [style=none] (86) at (-5.075, 3.925) {};
		\node [style=none] (87) at (-5.075, 4.075) {};
		\node [style=none] (88) at (4.575, 4.075) {};
		\node [style=none] (89) at (1.575, 2.075) {};
		\node [style=none] (90) at (-4.825, 2.925) {};
		\node [style=none] (91) at (-4.825, 3.075) {};
		\node [style=none] (92) at (1.825, 3.075) {};
		\node [style=none] (93) at (-4, 4.5) {{\tiny $\nabla_0$}};
		\node [style=none] (94) at (-1.525, 4.5) {{\tiny $\nabla_1$}};
		\node [style=none] (95) at (0.975, 4.5) {{\tiny $\nabla_2$}};
		\node [style=none] (96) at (3.475, 4.5) {{\tiny $\nabla_3$}};
		\node [style=none] (97) at (-6.5, 4.5) {{\tiny Depth}};
		\node [style=none] (98) at (-6.5, 4) {};
		\node [style=none] (99) at (-6.5, 3) {};
		\node [style=none] (100) at (-6.5, 2) {};
		\node [style=none] (101) at (-6.5, 1) {};
		\node [style=none] (102) at (-6.5, 0) {};
		\node [style=none] (103) at (-6.5, 0) {{\tiny $0$}};
		\node [style=none] (104) at (-6.5, 1) {{\tiny $1$}};
		\node [style=none] (105) at (-6.5, 2) {{\tiny $2$}};
		\node [style=none] (106) at (-6.5, 3) {{\tiny $3$}};
		\node [style=none] (107) at (-6.5, 4) {{\tiny $4$}};
		\node [style=none] (108) at (6, 2) {$\cdots$};
		\node [style=none] (109) at (3, -1.5) {$\cdots$};
		\node [style=none] (111) at (5.15, 3.5) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [style=semithick] (0) to (2);
		\draw [style=semithick] (2) to (4);
		\draw [style=semithick] (0) to (4);
		\draw [style=semithick] (5) to (6);
		\draw [style=semithick] (6) to (7);
		\draw [style=semithick] (5) to (7);
		\draw [style=semithick] (8) to (9);
		\draw [style=semithick] (9) to (10);
		\draw [style=semithick] (8) to (10);
		\draw [style=semithick] (11) to (12);
		\draw [style=semithick] (12) to (13);
		\draw [style=semithick] (11) to (13);
		\draw [style=semithick] (2) to (17);
		\draw [style=semithick] (17) to (6);
		\draw [style=semithick] (17) to (9);
		\draw [style=semithick] (17) to (12);
		\draw [style=semithick] (23) to (24);
		\draw [style=semithick] (27) to (28);
		\draw [style=semithick] (29) to (30);
		\draw [style=semithick] (31) to (32);
		\draw [style=semithick] (33) to (34);
		\draw [style=semithick] (25) to (26);
		\draw [style=semithick] (35) to (36);
		\draw [style=semithick] (37) to (38);
		\draw [style=semithick] (39) to (40);
		\draw [style=semithick] (41) to (42);
		\draw [style=semithick] (43) to (44);
		\draw [style=semithick] (45) to (46);
		\draw [style=rounded corners very thin] (53.center)
			 to (59.center)
			 to (55.center)
			 to (58.center)
			 to (57.center);
		\draw [style=rounded corners very thin] (61.center)
			 to (62.center)
			 to (72.center)
			 to (73.center)
			 to (74.center);
		\draw [style=rounded corners very thin] (57.center)
			 to (60.center)
			 to (61.center);
		\draw [style=rounded corners very thin] (67.center)
			 to (66.center)
			 to (74.center);
		\draw [style=rounded corners very thin] (77.center)
			 to (78.center)
			 to (79.center);
		\draw [style=rounded corners very thin] (79.center)
			 to (80.center)
			 to (81.center)
			 to (82.center);
		\draw [style=rounded corners very thin] (85.center)
			 to (84.center)
			 to (83.center)
			 to (82.center);
		\draw [style=rounded corners arrow] (85.center)
			 to (86.center)
			 to (87.center)
			 to (88.center)
			 to (111.center);
		\draw [style=rounded corners very thin] (67.center)
			 to (68.center)
			 to (69.center)
			 to (89.center);
		\draw [style=rounded corners very thin] (89.center)
			 to (90.center)
			 to (91.center)
			 to (92.center)
			 to (77.center);
	\end{pgfonlayer}
\end{tikzpicture}

